Uncovering the First AGN Jets with AXIS

Jets powered by AGN in the early Universe ($z \gtrsim 6$) have the potential to not only define the trajectories of the first-forming massive galaxies but to enable the accelerated growth of their associated SMBHs. Under typical assumptions, jets could even rectify observed quasars with light seed formation scenarios; however, not only are constraints on the parameters of the first jets lacking, observations of these objects are scarce. Owing to the significant energy density of the CMB at these epochs capable of quenching radio emission, observations will require powerful, high angular resolution X-ray imaging to map and characterize these jets. As such, \textit{AXIS} will be necessary to understand early SMBH growth and feedback.

==> Definitions/journalnames.tex <==
\DeclareOption{ArXiv}{ 	    \gdef\@journal{ArXiv}	\gdef\@journalshort{ArXiv}	\gdef\@journalfull{ArXiv}	\gdef\@doiabbr{ArXiv}	}
